Two Hands Are Better Than One (up to constant factors)

We study the difference between the standard seeded model of tile self-assembly, and the "seedless" two-handed model of tile self-assembly. Most of our results suggest that the two-handed model is more powerful. In particular, we show how to simulate any seeded system with a two-handed system that is essentially just a constant factor larger. We exhibit finite shapes with a busy-beaver separation in the number of distinct tiles required by seeded versus two-handed, and exhibit an infinite shape that can be constructed two-handed but not seeded. Finally, we show that verifying whether a given system uniquely assembles a desired supertile is co-NP-complete in the two-handed model, while it was known to be polynomially solvable in the seeded model.

==> atam.tex <==
\subsection{The abstract tile assembly model (aTAM)}
\label{sec:atam-def}
In the aTAM \cite{RotWin00, Roth01,Winf98}, self-assembly begins with a \emph{seed assembly} $\sigma$ (typically
assumed to be finite and $\tau$-stable) and
proceeds asynchronously and nondeterministically, with tiles
adsorbing one at a time to the existing assembly in any manner that
preserves stability at all times.

An aTAM \emph{tile assembly system} (\emph{TAS}) is an ordered triple
$\mathcal{T} = (T, \sigma, \tau)$, where $T$ is a finite set of tile
types, $\sigma$ is a seed assembly with finite domain, and $\tau$ is
the temperature. An \emph{assembly sequence} in a TAS $\mathcal{T} = (T, \sigma, \tau)$ is
a (possibly infinite) sequence $\vec{\alpha} = ( \alpha_i \mid 0
\leq i < k )$ of assemblies in which $\alpha_0 = \sigma$ and each
$\alpha_{i+1}$ is obtained from $\alpha_i$ by the ``$\tau$-stable''
addition of a single tile. The \emph{result} of an assembly sequence
$\vec{\alpha}$ is the unique assembly $\res{\vec{\alpha}}$
satisfying $\dom{\res{\vec{\alpha}}} = \bigcup_{0 \leq i <
k}{\dom{\alpha_i}}$ and, for each $0 \leq i < k$, $\alpha_i
\sqsubseteq \res{\vec{\alpha}}$.

We write $\prodasm{T}$ for the
\emph{set of all producible assemblies of} $\mathcal{T}$. An
assembly $\alpha$ is \emph{terminal}, and we write $\alpha \in
\termasm{\mathcal{T}}$, if no tile can be stably added to it. We
write $\termasm{T}$ for the \emph{set of all terminal assemblies of
} $\mathcal{T}$. A TAS ${\mathcal T}$ is \emph{directed}, or
\emph{produces a unique assembly}, if it has exactly one terminal
assembly i.e., $|\termasm{T}| = 1$. The reader is cautioned that the
term ``directed'' has also been used for a different, more specialized
notion in self-assembly \cite{AKKRS09}. We interpret ``directed'' to
mean ``deterministic'', though there are multiple senses in which a
TAS may be deterministic or nondeterministic.

Given a connected shape $X \subseteq \Z^2$,  we say a TAS $\calT$ \emph{self-assembles $X$} if every producible, terminal assembly places tiles exactly on those positions in $X$.  (Note that this notion is equivalent to \emph{strict} self-assembly as defined in \cite{jSSADST}.)  For an infinite shape $X \subseteq \Z^2$, we say that $\calT$ \emph{finitely self-assembles} $X$ if every finite producible assembly of $\mathcal{T}$ has a possible way of growing into an assembly that places tiles exactly on those points in $X$. Note that if a shape $X$ self-assembles in $\mathcal{T}$, then $X$ infinitely self-assembles in $\mathcal{T}$ (but not necessarily vice versa - see Figure~\ref{fig:fsa_vs_sa} for an example). 

==> tvp_2ham_temp1_algorithm.tex <==
For the terminality verification problem, we are given a 2HAM TAS $\mathcal{T} = (T,1)$ and an assembly $\alpha \in \prodasm{T}$ and we must decide whether or not $\alpha \in \termasm{T}$. We can accomplish this task in time $O(|\alpha||T|)$ by performing the following test. Check, for each $\vec{x} \in \dom{\alpha}$ and each $t \in T$, whether or not $t$ can bind to $\alpha$ at location $\vec{x}$. If any test passes, then we reject $\alpha$. Otherwise, if all tests fail, then we can accept $\alpha$. To see that such a test is sufficient, consider the fact that, at temperature $\tau = 1$, if $\alpha$ is not terminal, then there must be some assembly $\alpha' \in \prodasm{T}$ such that it is possible to combine $\alpha$ with $\alpha'$ to get $\alpha'' \in \prodasm{T}$. Since $\alpha'' \in \prodasm{T}$, there must be some position, say $\vec{y} \in \dom{\alpha''}$ such that $\vec{y} \in \dom{\alpha'}$ and $\alpha(\vec{y})$ interacts with some tile at position $\vec{z} \in \dom{\alpha}$. This means it would be possible to attach only the tile type $\alpha''(\vec{y})$ to $\alpha$ at location $\vec{z}$  since it would bind with positive strength. 

Noting that the perimeter of $\alpha$ is $O(|\alpha|)$ yields the desired time bound.  

==> tvp_2ham_temp2_impossible.tex <==
Let $H = \{ M \mid M \textmd{ halts on input } \lambda \}$. It suffices to exhibit a many-one reduction from $H$ to the terminality verification problem for 2HAM at temperature $t \geq 2$. Let $M$ be a Turing machine. The problem of simulating a Turing machine (on some input string) in the aTAM is a well-studied problem \cite{Winf98,RotWin00,jSADS,jCCSA}. Thus, let $\mathcal{T}_M = \left(T_M,\sigma_{\lambda},2\right)$ be an aTAM TAS, which is singly-seeded at the origin, directed, and such that $\mathcal{T}$ simulates $M$ on the empty string $\lambda$ in the most natural way. Let $\hat{t} \in T_M$ be the unique tile type such that $\hat{t}$ represents the state of $M$ if/when it ever reaches the halting state.

By Theorem~\ref{thm:sim_atam_1_2_with_2ham_at_2}, there exists a 2HAM TAS $\mathcal{S} = (S,2)$ that simulates $\mathcal{T} = (T,\sigma,2)$. The output of our reduction is the assembly $\widehat{\alpha} \in \prodasm{S}$ such that $R\left(\widehat{\alpha}\right) = \hat{t}$, i.e., the assembly in $\mathcal{S}$ that represents the halting tile in $T_M$.

If $M \in H$, then $M$ halts on $\lambda$ and $\mathcal{T}$ will place $\hat{t}$. This means that in the simulating system $\mathcal{S}$, the producible assembly $\widehat{\alpha}$ is not terminal. However, if $M \not \in H$, then $M$ never halts and $\mathcal{T}$ will never place $\hat{t}$, whence the assembly $\widehat{\alpha} \in \termasm{S}$. 



==> upv_is_in_co_np.tex <==
It suffices to show that if an instance of the unique producibility verification (UPV) is false, i.e., if the tile system in the instance does not assemble uniquely into the given assembly, then there is a short proof of the fact. By definition, a given 2HAM TAS $\mathcal{T} = (T,\tau)$ does not uniquely assemble into a given assembly $\alpha$ if and only if one of the following occurs:

\textbf{Case 1.} $\alpha \not \in \prodasm{T}$, which we can verify in polynomial time \cite{CarnivalGlass}.

\textbf{Case 2.} There exists $\widehat{\alpha} \in \termasm{T}$ such that $\widehat{\alpha} \ne \alpha$. Then $\widehat{\alpha}$, along with the order in which the tiles join to assemble $\widehat{\alpha}$ would suffice as a proof. In order to check this proof, we first verify that $\widehat{\alpha} \in \prodasm{T}$, which can be accomplished in polynomial time \cite{CarnivalGlass}. If $\widehat{\alpha} \not \in \prodasm{T}$, then we can reject this instance, so assume that $\widehat{\alpha} \in \prodasm{T}$. Since $\widehat{\alpha} \ne \alpha$, it must be the case that $\widehat{\alpha} \sqsubseteq \alpha$ because otherwise we could have rejected as we were building $\widehat{\alpha}$. Finally, we call attention to the fact that, if $\widehat{\alpha} \sqsubseteq \alpha$, then $\widehat{\alpha} \not \in \termasm{T}$ \cite{CarnivalGlass}, whence we can reject this instance.

\textbf{Case 3.} There exists $\widehat{\alpha} \in \prodasm{T}$ such that $\left| \widehat{\alpha} \right| > |\alpha|$, i.e., it is possible for $\mathcal{T}$ to produce some assembly that is strictly larger than $\alpha$. Note that it need not be the case that $\widehat{\alpha} \in \termasm{T}$ for our verification to work properly. If $\widehat{\alpha}$ exists, then there exists $\widehat{\alpha}'$ with $\left| \widehat{\alpha}' \right| \leq 2|\alpha|$ (in the worst case, two assemblies of size $|\alpha|$ could come together). Such an assembly $\widehat{\alpha}'$ along with the order in which assemblies are combined to assemble $\widehat{\alpha}'$ would suffice as a proof, which we can verify in polynomial time \cite{CarnivalGlass}. After we assemble $\widehat{\alpha}'$, we can verify that it is larger than $\alpha$.

In every case, the size of the proof is polynomial in the instance size and the verification always runs in polynomial time in the instance size.

